SepLL: Separating Latent Class Labels from Weak Supervision Noise

In the weakly supervised learning paradigm, labeling functions automatically assign heuristic, often noisy, labels to data samples. In this work, we provide a method for learning from weak labels by separating two types of complementary information associated with the labeling functions: information related to the target label and information specific to one labeling function only. Both types of information are reflected to different degrees by all labeled instances. In contrast to previous works that aimed at correcting or removing wrongly labeled instances, we learn a branched deep model that uses all data as-is, but splits the labeling function information in the latent space. Specifically, we propose the end-to-end model SepLL which extends a transformer classifier by introducing a latent space for labeling function specific and task-specific information. The learning signal is only given by the labeling functions matches, no pre-processing or label model is required for our method. Notably, the task prediction is made from the latent layer without any direct task signal. Experiments on Wrench text classification tasks show that our model is competitive with the state-of-the-art, and yields a new best average performance.

==> auxiliaries/notes.tex <==
Add the following related work:

Look at answers from reviews for related work

Andi does these two:

Named Entity Recognition without Labelled Data: A Weak Supervision Approach
P Lison, A Hubin, J Barnes, S Touileb https://arxiv.org/abs/2004.14723
=> they also predict Lf matches from latent classes, see Sec. 3.2

Feature-Dependent Confusion Matrices for Low-Resource NER Labeling with Noisy Labels
Lukas Lange, Michael A Hedderich, Dietrich Klakow https://www.aclweb.org/anthology/D19-1362
=> they also learn with a transition matrix from true (latent) labels to weak labels


Vasiliki:


[1] Xiao, Tong, et al. "Learning from massive noisy labeled data for image classification." In Proc. of CVPR. 2015.

[2] Goldberger, Jacob, and Ehud Ben-Reuven. "Training deep neural-networks using a noise adaptation layer." In Proc. ICLR 2016.

[3] X. Chen and A. Gupta, "Webly supervised learning of convolutional networks,” in Proc. ICCV, 2015, pp. 1431–1439.

[4] S. Sukhbaatar, J. Bruna, M. Paluri, L. Bourdev, and R. Fergus,
"Training convolutional networks with noisy labels,” in Proc. ICLRW,
2015, pp. 1–11.

[5] A. J. Bekker and J. Goldberger, "Training deep neural-networks based on unreliable labels,” in Proc. ICASSP, 2016, pp. 2682–2686.

==> auxiliaries/symbols_for_model_figure.tex <==


\begin{align*}
    f_{\hat{Y}} \\
    f_{\hat{L}} \\
    f_{\Tilde{Y}} \\
    f_{\Tilde{L}} \\
    f_{L} \\
    L \\
    Y \\
    \hat{L} \\
    \hat{Y} \\
    \Tilde{L} \\
    \Tilde{Y} \\
    Z
    \\
    X \\
    \mathcal{L} \\
    h
\end{align*}

==> chapters/discussion.tex <==

\section{Discussion}

This work stands in contrast to the current path weak supervision is going.
While it shares the idea to use the three pillars of weak labeling matches, label-class relation and pre-trained transformer, 
we disagree on how to use the them.
Now,  label / end model and teacher-student models seem to be the common line of research.

==> files/algorithm.tex <==
\begin{algorithm}[t]
    \caption{\algname{}}
    \begin{algorithmic}
    \Require BERT-based encoder
        
        \State \COMMENT{\# \textbf{Clustering Stage}}
        \For{ Mini batch $B=(X, L) \in \mathbb{R} \times \mathbb{R}^{n \times m}$ }
            \State Run encoder $Z=h(X)$
            \State Compute latent spaces $L_\hat{L}$
            \State Compute labeling function distribution $Q=$
            \State Compute loss $\mathcal{L}=\dots$
        \EndFor
        
        \end{algorithmic}
        \label{alg:ach}
        \end{algorithm}

==> files/cosine_results_table.tex <==

\begin{table*}
    \centering
    \begin{tabular}{lrrrrrrrrr}
\toprule
            &  IMDb &  Yelp &  Youtube &   SMS &  AGNews &  Trec & Spouse &  Semeval &      Avg. \\
\midrule
     Gold+Roberta & 93.25 & 97.13 &    95.68 & 96.31 &   91.39 & 96.68 &      - &    93.23 & 87.96 \\
               \hline
 MV+CosineRoberta & \textbf{88.22} & 94.23 &    \textbf{97.60} & 96.67 &   \textbf{88.15} & 77.96 &   \textit{40.5} &    86.20 & 83.69 \\
 DP+CosineRoberta & 87.91 & 94.09 &    96.80 & 31.71 &   87.53 & 82.36 &  28.86 &    75.17 & 73.05 \\
  LF\_split+COSINE & 88.00 & \textbf{95.07} &    \textbf{97.60} & \textbf{97.04}&   85.47 & \textbf{83.20} &  \textbf{43.2} &  \textbf{86.83} & \textbf{84.47} \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:results_cosine}
\end{table*}

==> files/hyperparam_table.tex <==
\begin{table}
    \centering
\begin{tabular}{lr}
\toprule
          Model & hyperparameter & values \\
          
\midrule
    Full Model & 83.14 \\
\bottomrule
\end{tabular}
\caption{Ablation of information routing strategies. Each strategy is removed individually. The basic model does not use any strategy.}
\label{tab:ablation_small}
\end{table}


==> files/lf_match_prediction_table.tex <==
\begin{table}
    \centering
\begin{tabular}{lrr}
\toprule
 dataset &   acc &    f1 \\
\midrule
    imdb & 90.20 & 89.41 \\
    yelp & 91.47 & 89.52 \\
 youtube & 82.88 & 76.49 \\
     sms & 96.43 & 97.61 \\
    trec & 99.41 & 99.41 \\
  spouse & 95.92 & 94.51 \\
 semeval & 99.46 & 99.51 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:lf_preds}
\end{table}

==> files/lf_match_prediction_train_table.tex <==
\begin{table*}
    \centering
\begin{tabular}{lrrrrrrrrrr}
\toprule
 dataset &  latent acc &   acc &  y\_acc &  latent f1 &    f1 &  y\_f1 &  latent ce &   ce &  y\_ce &  uni\_ce \\
\midrule
    imdb &       90.30 & 90.24 &  86.89 &      89.51 & 89.58 & 80.79 &       1.43 & 1.41 &  2.12 &    2.20 \\
    yelp &       91.67 & 91.67 &  90.22 &      89.63 & 89.65 & 85.58 &       2.20 & 2.15 &  2.61 &    2.71 \\
 youtube &       85.43 & 86.25 &  83.66 &      80.62 & 82.41 & 76.21 &       1.66 & 1.63 &  2.13 &    2.30 \\
     sms &       96.47 & 95.79 &  99.28 &      97.65 & 97.28 & 98.93 &       4.08 & 4.91 &  4.53 &    4.29 \\
  agnews &       91.62 & 92.02 &  89.66 &      89.92 & 91.14 & 84.77 &       1.67 & 1.60 &  1.91 &    2.20 \\
    trec &       99.35 & 99.21 &  94.84 &      99.35 & 99.22 & 95.45 &       1.25 & 1.19 &  3.58 &    4.22 \\
  spouse &       96.38 & 96.70 &  96.25 &      95.21 & 96.41 & 94.41 &       2.03 & 2.01 &  2.15 &    2.20 \\
 semeval &       99.55 & 98.47 &  92.75 &      99.59 & 98.84 & 95.58 &       1.41 & 0.94 &  3.21 &    5.10 \\
 average &       93.85 & 93.79 &  91.69 &      92.68 & 93.07 & 88.96 &       1.97 & 1.98 &  2.78 &    3.15 \\
\bottomrule
\end{tabular}

    \caption{Train set}
    \label{tab:lf_preds_train_full}
\end{table*}
